A termination criterion for stochastic gradient descent for binary classification

We propose a new, simple, and computationally inexpensive termination test for constant step-size stochastic gradient descent (SGD) applied to binary classification on the logistic and hinge loss with homogeneous linear predictors. Our theoretical results support the effectiveness of our stopping criterion when the data is Gaussian distributed. This presence of noise allows for the possibility of non-separable data. We show that our test terminates in a finite number of iterations and when the noise in the data is not too large, the expected classifier at termination nearly minimizes the probability of misclassification. Finally, numerical experiments indicate for both real and synthetic data sets that our termination test exhibits a good degree of predictability on accuracy and running time.

==> arxiv_hinge_loss.tex <==
\subsection{Hinge Regression}
In this section, we study the following optimization problem
\begin{align*}
   \min f(\btheta):=\bE_{\bxi \sim \mathcal{P}_*} [\ell(\bxi^T\btheta)],
\end{align*}
where $\ell(x):=\ell(x,1)$ with the hinge loss function defined in \eqref{eq:hinge_loss_definition}.  We state the main theorem of this section below. We defer the proof to the end of this subsection. 

\begin{theorem}\label{theorem_hinge}
Let $\btheta_0=\bm{0}$. The following are true.
\begin{enumerate}
    \item  Fix $\epsilon\in (0,\tfrac{1}{2})$ and let $M=1+\frac{\alpha(\Vert \bmu \Vert^2+\sigma^2)}{2\epsilon}$. Suppose that $\sigma \leq \left(\tfrac{1}{2}-\epsilon\right)\sqrt{\tfrac{\pi}{2}}\Vert \bmu \Vert$ (low variance regime). The following then holds. 
\begin{equation}\begin{aligned} \label{eq:low_Et_proof}
\bE[T]&\leq \left(2+\frac{\left(M-1\right)^2}{\alpha\Vert \bmu \Vert^2}+\frac{\sigma}{\Vert \bmu \Vert}\left(\frac{1.6M^2}{\alpha \Vert \bmu \Vert^2}+7,612\sigma^2\alpha^4\Vert\bmu \Vert^4\right) \right)+\frac{2M^2}{\alpha \Vert\bmu\Vert^2}.
\end{aligned} \end{equation}  
\item Suppose that $\sqrt{\frac{\pi}{8}}\Vert \bmu \Vert \leq \sigma$ (high variance regime).  It holds that $\bE[T]<+\infty$ provided the step-size $\alpha$ satisfies
\begin{equation}
    \alpha< \frac{\min\{1,\tfrac{1}{2}r\rho^*\}}{\Vert \bmu \Vert^2+d\sigma^2}
\end{equation}
where the constant $r$ is defined as 
\begin{equation*}
    r:= \frac{64}{125 \rho^*\sigma \Vert \bmu \Vert \sqrt{2\pi}}\exp\left(-\frac{(\tfrac{4}{3}\frac{1}{\rho^*}-\Vert \bmu \Vert^2)^2}{2\sigma^2\Vert \bmu \Vert^2} \right).
\end{equation*}
\end{enumerate}
  \end{theorem}

\subsubsection{Low Variance Regime}\label{sec:low_hinge}
Throughout this section, we fix a positive constant $0<\epsilon<\tfrac{1}{2}$ and consider the following drift function. 
\[
V(\btheta):=\frac{1}{\alpha \Vert \bmu\Vert^2}(M-\bmu^T\btheta)^2,
\]
where $M=1+\frac{\alpha(\Vert \bmu \Vert^2+\sigma^2)}{2\epsilon}$. In addition, we consider the following target set. 
\begin{equation}\label{eq:hinge_low_C}
    C:=\{\btheta:\bmu^T\btheta \geq 1\}.
\end{equation}
\begin{proposition}\label{prop:low_noise_hinge_Etau1}
Fix $\epsilon\in(0,\tfrac{1}{2})$ and suppose that $\sigma \leq \left(\tfrac{1}{2}-\epsilon\right)\sqrt{\tfrac{\pi}{2}}\Vert \bmu \Vert$. Let $\btheta\in \R^d$ such that $\bmu^T\btheta\leq 1$. The following is then true 
\begin{equation}
    \bE[\tau_1^C|\btheta_0=\btheta]\leq V(\btheta).
\end{equation}
\end{proposition}
\begin{proof}

Suppose that $\bmu^T\btheta_{k-1}\leq 1$. It, then, holds that 
\begin{align}
    \bE[(M-\bmu^T\btheta_k)^2|\mathcal{F}_{k-1}]1_{\{\tau_1^C\wedge n\geq k \}}&= \bE_{\bxi_k}[(M-\bmu^T\btheta_{k-1}-\alpha 1_{\{\bxi_k^T\btheta_{k-1}\leq 1\}}\bmu^T\bxi_k)^2|\mathcal{F}_{k-1}]1_{\{\tau_1^C\wedge n\geq k \}}\\&=(M-\bmu^T\btheta_{k-1})^2-2\alpha(M-\bmu^T\btheta_{k-1})\bE_{\bxi_k}[1_{\{\bxi_k^T\btheta_{k-1}\leq 1\}}\bmu^T\bxi_k|\mathcal{F}_{k-1}]\\&+\alpha^2\bE_{\bxi_k}[1_{\{\bxi_k^T\btheta_{k-1}\leq 1\}}(\bmu^T\bxi_k)^2|\mathcal{F}_{k-1}].
\end{align}
We need to lower bound the quantity $\bE_{\bxi_k}[1_{\{ \bxi_k^T\btheta_{k-1}\leq 1\}}\bmu^T\bxi_k|\mathcal{F}_{k-1}]$. We have 
\begin{align}
    \bE_{\bxi_k}[1_{\{ \bxi_k^T\btheta_{k-1}\leq 1\}}\bmu^T\bxi_k|\mathcal{F}_{k-1}]&=\Vert \bmu\Vert^2\bE_{\bxi_k}[1_{\{ \bxi_k^T\btheta_{k-1}\leq 1\}}|\mathcal{F}_{k-1}]+\bE_{\bxi_k}[1_{\{ \bxi_k^T\btheta_{k-1}\leq 1\}}\bmu^T(\bxi_k-\bmu)|\mathcal{F}_{k-1}]\\&\geq \tfrac{1}{2}\Vert \bmu \Vert^2-\bE_{\bxi_k}[\vert \bmu^T(\bxi_k-\bmu)]\vert]\\&\geq \tfrac{1}{2}\Vert \bmu \Vert^2-\sqrt{\tfrac{2}{\pi}}\sigma\Vert \bmu \Vert. 
\end{align}
Here we used that $1_{\{\bxi_k^T\btheta_{k-1}\leq \bmu^T\btheta_{k-1}\}}\leq 1_{\{\bxi_k^T\btheta_{k-1}\leq 1\}}$ and  $\bE_{\bxi_k}[1_{\{\bxi_k^T\btheta_{k-1}\leq \bmu^T\btheta_{k-1}\}}]=\tfrac{1}{2}$. Continuing, we obtain that 
\begin{align*}
\bE[(M-\bmu^T\btheta_k)^2-(M-\bmu^T\btheta_{k-1})^2&|\mathcal{F}_{k-1}]1_{\{\tau_1^C\wedge n\geq k \}}\\
&\leq \alpha^2 \bE_{\bxi_k}[(\bmu^T\bxi_k)^2]-2\alpha(M-\bmu^T\btheta_{k-1})(\tfrac{1}{2}\Vert \bmu \Vert^2-\sqrt{\tfrac{2}{\pi}}\sigma\Vert \bmu \Vert)\\&\leq \alpha^2\Vert \bmu\Vert^2(\Vert \bmu \Vert^2+\sigma^2)-2\alpha(M-\bmu^T\btheta_{k-1})\left(\tfrac{1}{2}\Vert \bmu \Vert^2-\sqrt{\tfrac{2}{\pi}}\sigma\Vert \bmu \Vert\right)
\end{align*}
Hence, using the bounds $
\sigma\leq \left(\tfrac{1}{2}-\epsilon\right)\sqrt{\tfrac{\pi}{2}}\Vert \bmu \Vert$ and $M\geq 1+\frac{\alpha(\Vert \bmu \Vert^2+\sigma^2)}{2\epsilon}$, we obtain that
\begin{align*}
    \bE[V(\btheta_k)-V(\btheta_{k-1})|\mathcal{F}_{k-1}]1_{\{\tau_1^C\wedge n\geq k \}}\leq \alpha (\Vert \bmu \Vert^2+\sigma^2)-2(M-\bmu^T\btheta_{k-1})\left(\tfrac{1}{2}-\sqrt{\tfrac{2}{\pi}}\frac{\sigma}{\Vert \bmu \Vert}\right)\leq -1_{\{\tau_1^C\wedge n\geq k \}}.
\end{align*}

Using Appendix Lemma \ref{lem:drift_lemma_appendix}, we obtain that $\bE[\tau_1^C\wedge n|\mathcal{F}_{-1}] \leq V(\btheta)$. Monotone convergence theorem completes the proof.
\end{proof}
We next upper bound the expected value of $\tau_m^C$ when we initialize with $\btheta_0=\bm{0}$.
\textcolor{red}{Is the proof of this proposition the same as Proposition 2 in logistic} 
\textcolor{blue}{Sina:They have a lot in common! but not entirely the same. It would be best if we make this one shorter.}
\begin{proposition}\label{prp:hinge_low_etm}
Let $\btheta_0=\bm{0}$ and suppose that $\sigma\leq \left(\tfrac{1}{2}-\epsilon\right)\sqrt{\tfrac{\pi}{2}}\Vert \bmu \Vert$. Consider the set $C$ defined in \eqref{eq:hinge_low_C}. Then the following bound holds for all $m \ge 1$
\begin{equation}
   \bE[\tau_m^C]\leq (m-1)\left(2+\frac{\left(M-1\right)^2}{\alpha\Vert \bmu \Vert^2}+\frac{\sigma}{\Vert \bmu \Vert}\left(\frac{1.6M^2}{\alpha \Vert \bmu \Vert^2}+7,612\sigma^2\alpha^4\Vert\bmu \Vert^4\right) \right)+\frac{M^2}{\alpha \Vert\bmu\Vert^2},
\end{equation}
where $M=1+\frac{\alpha(\Vert \bmu \Vert^2+\sigma^2)}{2\epsilon}$.
\end{proposition}

\begin{proof}
Similar to \eqref{eq: low_noise_bound}, we obtain that 
\begin{equation}\label{eq:low_noise_hinge1}
    \bE\left[(\tau_m^{C}-\tau_{m-1}^{C})\wedge n|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]\leq 2+\sum_{i=1}^{\infty}\bE\left[\tau_1^{C}\wedge n|\btheta_0=\btheta_{\tau_{m-1}^{C}+1}\right]1_{\{i-1\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}<i\}}. 
\end{equation}
For each $i \ge 2$, we observe the bound
\begin{align*}
    i-1 \leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1} &=1-\bmu^T\btheta_{\tau_{m-1}^{C}}-\alpha \bmu^T\bxi_{\tau_{m-1}^C+1}1_{\{\bxi_{\tau_{m-1}^C+1}^T\btheta_{\tau_{m-1}^C}\leq 1\}}\\&\leq -\alpha \bmu^T\bxi_{\tau_{m-1}^C+1}1_{\{\bxi_{\tau_{m-1}^C+1}^T\btheta_{\tau_{m-1}^C}\leq 1\}}\\&\leq -\alpha \bmu^T\bxi_{\tau_{m-1}^C+1}.
    \end{align*}
    Here the first inequality follows since $1\leq \bmu^T\btheta_{\tau_{m-1}^C}$ and the second inequality from the fact that $0\leq -\alpha \bmu^T\bxi_{\tau_{m-1}^C+1}$ as $i-1> 0$. We next, similar to our computation in \eqref{eq: low_noise_blah_3} and \eqref{eq: low_noise_blah_4}, have that 
    \begin{equation} \begin{aligned}  \label{eq: low_noise_hinge2}
\bE\left[\tau_1^{C}\wedge n|\btheta_0=\btheta_{\tau_{m-1}^{C}+1}\right]1_{\{i-1\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}<i\}}&\leq  \frac{(M+i-1)^2}{\alpha \Vert \bmu\Vert^2}1_{\{ \bmu^T\bxi_{\tau_{m-1}^{C}+1}\leq \frac{1-i}{\alpha}\}} \quad \forall i\geq 2.
\end{aligned} \end{equation}
Moreover, 
\begin{equation} \begin{aligned} \label{eq: low_noise_hinge_3}
    \bE\left[1_{\{ \bmu^T\bxi_{\tau_{m-1}^{C}+1}\leq \frac{1-i}{\alpha}\}} \right]&=\Phi\left(\frac{\frac{1-i}{\alpha}-\Vert \bmu\Vert^2}{\sigma\Vert \bmu\Vert } \right).
\end{aligned} \end{equation}
Combining \eqref{eq:low_noise_hinge1}, \eqref{eq: low_noise_hinge2} and \eqref{eq: low_noise_hinge_3} we obtain that 
\begin{equation}\label{eq:low_noise_hinge_blah12}
    \bE\left[(\tau_m^{C}-\tau_{m-1}^{C})\wedge n|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]\leq 2+\frac{\left(M-1\right)^2}{\alpha\Vert \bmu \Vert^2}+\frac{\sigma}{\Vert \bmu \Vert\sqrt{2\pi}}\sum_{i=2}^{+\infty}\frac{\left(M+i-1\right)^2}{\alpha \Vert \bmu \Vert^2+i-1}\exp\left(-\tfrac{1}{2}\left(\frac{\Vert \bmu \Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu \Vert^2}\right)^2 \right).
\end{equation}
Note that we used the bound $\bE\left[\tau_1^{C}\wedge n|\btheta_0=\btheta_{\tau_{m-1}^{C}+1}\right]1_{\{0\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}<1\}}\leq \frac{(M-1)^2}{\alpha \Vert\bmu\Vert^2}$. Continuing, similar to \eqref{eq: low_noise_blah_6} and \eqref{eq: low_noise_blah_7}, we have 
\begin{equation}
    \sum_{i=3}^{+\infty}\frac{\left(M+i-1\right)^2}{\alpha \Vert \bmu \Vert^2+i-1}\exp\left(-\tfrac{1}{2}\left(\frac{\Vert \bmu \Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu \Vert^2}\right)^2 \right) \leq 19,080 \alpha^4 \sigma^4 \Vert \bmu \Vert^4.
\end{equation}
We upper bound the term in \eqref{eq:low_noise_hinge_blah12} for $i=2$ by $\frac{4M^2}{\alpha \Vert \bmu \Vert^2}$. Finally we conclude that 
\begin{equation}
    \bE\left[\tau_m^C-\tau_{m-1}^C\wedge n \right] \leq 2+\frac{\left(M-1\right)^2}{\alpha\Vert \bmu \Vert^2}+\frac{\sigma}{\Vert \bmu \Vert}\left(\frac{1.6M^2}{\alpha \Vert \bmu \Vert^2}+7,612\sigma^2\alpha^4\Vert\bmu \Vert^4\right). 
\end{equation}
We, therefore, obtain that 
\begin{equation}
    \bE\left[\tau_m^C\right] \leq (m-1)\left(2+\frac{\left(M-1\right)^2}{\alpha\Vert \bmu \Vert^2}+\frac{\sigma}{\Vert \bmu \Vert}\left(\frac{1.6M^2}{\alpha \Vert \bmu \Vert^2}+7,612\sigma^2\alpha^4\Vert\bmu \Vert^4\right) \right)+\bE\left[\tau_1^C\right]
\end{equation}
The result follows after applying Proposition \ref{prop:low_noise_hinge_Etau1} with $\btheta_0=\bm{0}$. 
  \end{proof} 


 \begin{proof}[Proof of Theorem 3.1] Using Proposition \ref{prp:hinge_low_etm} and Lemma \ref{lem:stopping_time_appendix}, Theorem \ref{theorem_hinge}.1 immediately follows.
 \end{proof}

\subsubsection{High Variance Regime}\label{sec:high_hinge}
The main theorem of this section is as follows. 
\begin{theorem}\label{thm:hinge_loss_high_noise}
Suppose that the step-size $\alpha$ satisfies 
\begin{equation}
    \alpha< \frac{\min\{1,\tfrac{1}{2}r\rho^*\}}{\Vert \bmu \Vert^2+d\sigma^2}
\end{equation}
where $\rho^*$ is defined in Lemma \ref{lem:hinge_minimizer} and the constant $r$ is defined as 
\begin{equation*}
    r:= \frac{64}{125 \rho^*\sigma \Vert \bmu \Vert \sqrt{2\pi}}\exp\left(-\frac{(\tfrac{4}{3}\frac{1}{\rho^*}-\Vert \bmu \Vert^2)^2}{2\sigma^2\Vert \bmu \Vert^2} \right).
\end{equation*}
Then it holds that $\bE[T]<+\infty$. 
\end{theorem}
We refer the proof to the end of this section. We first need a technical lemma. 
\begin{lemma}\label{lem:hinge_loss_high_noise_fundamental_lemma}
For any $\btheta$ the following holds
\begin{equation}\label{eq:lemma_for_high_noise_hinge}
    f(\btheta_{k-1})-f(\btheta) \leq \frac{1}{2\alpha} \left(\Vert \btheta_{k-1}-\btheta\Vert^2-\bE\left[\Vert \btheta_k-\btheta\Vert^2 |\mathcal{F}_{k-1}\right]\right)+\frac{\alpha}{2}\left(\Vert \bmu \Vert^2+d\sigma^2\right).
\end{equation}
\end{lemma}
\begin{proof}
See Appendix, Lemma \ref{lem:technical_convex_bound}. Note that we are using the inequality $\Vert \nabla_{\btheta}\ell(\bxi^T\btheta)\Vert^2\leq \Vert \bxi \Vert^2$ and then applying \eqref{fact:norm_Gaussians}.
\end{proof}
We write the orthogonal complement of $\btheta\in \R^d$ as $\btheta=\rho\bmu+\tilde{\btheta}$. As before, the idea is to lower bound the left hand side of \eqref{eq:lemma_for_high_noise_hinge} for $\btheta=\btheta^*:=\rho^* \bmu$. To do so, we write $f(\btheta_{k-1})-f(\btheta^*)=f(\btheta_{k-1})-f(\rho\bmu)+f(\rho \bmu)-f(\btheta^*)$ and then provide bounds for the both terms $f(\btheta_{k-1})-f(\rho_{k-1} \bmu)$ and  $f(\rho_{k-1}\bmu)-f(\rho^*\bmu)$.
 The following lemma bounds $f(\btheta_{k-1})-f(\rho \bmu)$.
\begin{lemma}\label{lem:hinge_high_noise_first_lemma} For each $\btheta\in \R^d$, the following bound holds
\begin{equation}
   f(\btheta)-f(\rho\bmu)\geq \max\left\{\tfrac{1}{\sqrt{2\pi}}\sigma \Vert \tilde{\btheta}\Vert-\rho \Vert \bmu \Vert\left(\sigma\sqrt{\tfrac{2}{\pi}}+\Vert \bmu \Vert \right)-1,0 \right\}.
\end{equation}
\end{lemma}
\begin{proof} We begin by denoting
$\xi_1:=\bxi^T\tilde{\btheta}$ and $\xi_2:=\bxi^T\bmu$. Notice that $\xi_1$ and $\xi_2$ are independent random variables. We have that 
\begin{align*}
    f(\btheta)-f(\rho \bmu)&=\bE_{\bxi}\left[\ell(\bxi^T\btheta)-\ell(\rho\bxi^T\bmu) \right]\\&=\bE_{\bxi}\left[\ell(\xi_1+\rho\xi_2)-\ell(\rho\xi_2) \right]\\&=\bE_{\bxi}\left[\ell(-\xi_1+\rho\xi_2)-\ell(\rho\xi_2) \right].
\end{align*}
The second equality follows since $\xi_1 \sim -\xi_1$. We define the function 
\[
\Phi(\xi_1,\xi_2):=\ell(\xi_1+\rho\xi_2)+\ell(-\xi_1+\rho\xi_2)-2\ell(\rho\xi_2).
\] 
We, therefore, obtain that 
\[
2\left(f(\btheta)-f(\rho\bmu)\right)=\bE_{\xi_1,\xi_2}\left[\Phi(\xi_1,\xi_2)\right].
\]
We, next, claim that
\begin{equation}\label{eq:hinge_lemma_claim1}
    \Phi(\xi_1,\xi_2)=0 \text{ whenever } \vert \xi_1\vert\leq \vert 1-\rho\xi_2\vert.
\end{equation}
To see this, suppose that $\vert \xi_1\vert\leq \vert 1-\rho\xi_2\vert$ holds. We consider two cases.  First, assume that $0\leq 1-\rho\xi_2$. Then, it holds that $\rho\xi_2-\xi_1\leq 1$ and $\rho\xi_2+\xi_1\leq 1$. We then have $\Phi(\xi_1,\xi_2)=1-\xi_1-\rho\xi_2+1+\xi_1-\rho\xi_2-2(1-\rho\xi_2)=0$. Second, assume that $1-\rho\xi_2\leq 0$. Then, it holds that $1\leq \rho\xi_2-\xi_1$ and $1\leq \rho\xi_2+\xi_1$. Now it immediately follows that $\Phi(\xi_1,\xi_2)=0$. We have thus established \eqref{eq:hinge_lemma_claim1}. We, next, claim the following 
\begin{equation}\label{eq:hinge_lemma_claim2}
    \Phi(\xi_1,\xi_2)=\vert \xi_1\vert-\vert 1-\rho\xi_2\vert \text{ whenever } \vert \xi_1\vert\geq \vert 1-\rho\xi_2\vert.
\end{equation}
To this end, we again consider two cases. First, assume that $\xi_1\leq -\vert 1-\rho\xi_2\vert$. It, then, holds that $1\leq -\xi_1+\rho\xi_2$ and $\xi_1+\rho\xi_2\leq 1$. We, therefore, have $ \Phi(\xi_1,\xi_2)= 1-\xi_1-\rho\xi_2-2\ell(\rho\xi_2)$. The claim \eqref{eq:hinge_lemma_claim2} follows from the following simple identity 
\begin{equation}\label{eq:hinge_identity}
   2\ell(t)= 1-t+\vert 1 - t \vert, \quad \forall t \in \R.
\end{equation}
Second, assume that $\xi_1\geq \vert 1-\rho\xi_2\vert$. It, then, holds that $\xi_1+\rho\xi_2\geq 1$ and $-\xi_1+\rho\xi_2\leq 1$. We, therefore, have $
\Phi(\xi_1,\xi_2)=1+\xi_1-\rho\xi_2-2\ell(\rho \xi_2).
$ The claim \eqref{eq:hinge_lemma_claim2} follows from the identity \eqref{eq:hinge_identity}.  We, therefore, obtain 
\begin{align}
    \bE_{\xi_1,\xi_2}[\Phi(\xi_1,\xi_2)]&=2\bE_{\xi_1,\xi_2}[(\ell(\xi_1+\rho\xi_2)+\ell(-\xi_1+\rho\xi_2)-2\ell(\rho\xi_2))1_{\{ \xi_1>0\}}]\label{eq:hinge_lemma_it1}\\&=2\bE_{\xi_1,\xi_2}[(\ell(\xi_1+\rho\xi_2)+\ell(-\xi_1+\rho\xi_2)-2\ell(\rho\xi_2))1_{\{ \xi_1\geq\vert 1-\rho \xi_2\vert\}}]\label{eq:hinge_lemma_it2}\\&=\bE_{\xi_1,\xi_2}[(\xi_1-\vert 1-\rho \xi_2\vert)1_{\{ \xi_1\geq \vert 1-\rho\xi_2\vert\}} ]. \label{eq:hinge_lemma_it3}
\end{align}
Here, \eqref{eq:hinge_lemma_it1} holds because $\xi_1\sim -\xi_1$ and $\Phi(\xi_1,\xi_2)=\Phi(-\xi_1,\xi_2)$. Equation \eqref{eq:hinge_lemma_it2} is true because of claim \eqref{eq:hinge_lemma_claim1} and \eqref{eq:hinge_lemma_it3} follows from claim \eqref{eq:hinge_lemma_claim2}. From \eqref{eq:hinge_lemma_it3}, we clearly conclude that $\bE_{\xi_1,\xi_2}[\Phi(\xi_1,\xi_2)]\geq 0$.  We, next, observe the bound
\begin{align}
    \bE_{\xi_1,\xi_2}[(\xi_1-\vert 1-\rho \xi_2\vert)1_{\{ \xi_1\geq \vert 1-\rho\xi_2\vert\}} ] &= \tfrac{1}{2}\bE_{\xi_1,\xi_2}[\xi_1-\vert 1-\rho \xi_2\vert+\vert \xi_1-\vert 1-\rho \xi_2\vert \vert]\nonumber\\&\geq -\tfrac{1}{2}\bE_{\xi_2}[\vert 1-\rho \xi_2\vert]+\tfrac{1}{2}\bE_{\xi_1,\xi_2}[\vert \xi_1\vert-\vert 1-\rho \xi_2\vert]\nonumber\\&=\tfrac{1}{2}\bE_{\xi_1}[\vert \xi_1\vert]-\bE_{\xi_2}[\vert1-\rho\xi_2\vert]. \label{eq:thrid_last_equation}
\end{align}
The second inequality follows from $\bE_{\xi_1}[\xi_1]=0$ and the triangle inequality $\vert x\vert-\vert y\vert \leq \vert \vert x\vert-y\vert$. On the other hand, it holds that
\begin{equation}\label{first_last_equation}
\bE_{\xi_1}[\vert \xi_1\vert]=\sqrt{\tfrac{2}{\pi}}\sigma \Vert \tilde{\btheta}\Vert,
\end{equation}
and 
\begin{equation}\label{second_last_equation}
\bE_{\bxi}[\vert 1-\rho \bmu^T\bxi\vert]\leq 1+\rho \bE_{\bxi}[\vert \bmu^T\bxi\vert]\leq 1+\rho\Vert \bmu \Vert \left(\sigma \sqrt{\tfrac{2}{\pi}}+\Vert \bmu \Vert \right).
\end{equation}
Combing equations \eqref{eq:thrid_last_equation}
, \eqref{first_last_equation} and \eqref{second_last_equation} concludes the proof.
\end{proof}
In turn, we bound $f(\rho \bmu)-f(\rho^*\bmu)$ in the next lemma.
\begin{lemma}\label{lem:hinge_loss_second_lemma}
There exists a constant $r>0$ such that the following holds  
\begin{equation}
    f(\rho \bmu)-f(\rho^*\bmu) \geq r\vert \rho -\rho^*\vert \quad \text{for any $\rho$ satisfying $\vert \rho-\rho^*\vert >\tfrac{1}{2}\rho^*$ }.
\end{equation}
\end{lemma}
\begin{proof}
We begin by defining the function $h(\rho)=f(\rho\bmu)$. Recall that 
\[
f(\rho \bmu)=\bE_{\bxi \sim \mathcal{P}_*}[\ell(\rho\bxi^T\bmu)]=\bE_{\bxi \sim \mathcal{P}_*}[(1-\rho \bxi^T\bmu)1_{\{\rho\bxi^T\bmu\leq 1 \}}]
\]
Hence, it holds that 
\[
h'(\rho)=\bmu^T\nabla f(\rho \bmu)=-\bE_{\bxi \sim \mathcal{P}_*}[\bxi^T\bmu1_{\{ \rho\bxi^T\bmu\leq 1\}}].
\]
From \eqref{eq:fact_affine}, we obtain that $\bmu^T\bxi \sim N(\Vert \bmu \Vert^2,\sigma^2\Vert \bmu \Vert^2)$.  For $\rho>0$, therefore, it holds that
\begin{equation}\label{der_phi_pos}
    h'(\rho)=\frac{-1}{\sigma\Vert \bmu \Vert\sqrt{2\pi}}\int_{-\infty}^{\frac{1}{\rho}}z\exp\left(-\frac{(z-\Vert \bmu \Vert^2)^2)}{2\sigma^2\Vert \bmu \Vert^2} \right)dz.
\end{equation}
Applying chain rule thus yields 
\[
h''(\rho)=\frac{1}{\rho^3\sigma\Vert \bmu \Vert\sqrt{2\pi}}\exp\left(-\frac{(\frac{1}{\rho}-\Vert \bmu \Vert^2)^2}{2\sigma^2\Vert \bmu \Vert^2}  \right) \quad \text{for all $\rho>0$}.
\]
Clearly, there exists $r>0$ such that for $\rho\in [\tfrac{3}{4}\rho^*,\tfrac{5}{4}\rho^*]$, it holds that $h''(\rho)\geq r$. Applying Lemma \ref{lem:convex_analysis_lemma} the result follows with the constant $r$ defined as follows
\begin{equation}\label{eq:constant_r_hinge_loss}
    r:= \frac{64}{125 \rho^*\sigma \Vert \bmu \Vert \sqrt{2\pi}}\exp\left(-\frac{(\tfrac{4}{3}\frac{1}{\rho^*}-\Vert \bmu \Vert^2)^2}{2\sigma^2\Vert \bmu \Vert^2} \right).
\end{equation}
\end{proof}
We define the target set $C$ as follows:
\begin{equation}\label{target_set_for_hinge}
    C:=\left\{\btheta:\vert \rho-\rho^*\vert \leq \tfrac{1}{2}\rho^* \text{ and } \Vert \tilde{\btheta}\Vert \leq c:=\frac{\sqrt{2\pi}}{\sigma}\left(2+\tfrac{3}{2}\rho^*\Vert \bmu \Vert\left(\sigma\sqrt{\tfrac{2}{\pi}}+\Vert \bmu \Vert \right) \right) \right\}.
\end{equation}
Also, we consider the following drift function 
\begin{equation}
    V(\btheta):=\Vert \btheta -\btheta^*\Vert^2.
\end{equation}
The following proposition establishes the drift equation.
\begin{proposition}
Suppose that the step-size $\alpha$ satisfies the bound
\begin{equation}\label{bound_for_alpha_hinge_loss}
    \alpha< \frac{\min\{1,\tfrac{1}{2}r\rho^*\}}{\Vert \bmu \Vert^2+d\sigma^2}
\end{equation}
where $r$ is defined in \eqref{eq:constant_r_hinge_loss}. The following is then true. 
\begin{equation}
    \left(\bE\left[V(\btheta_k)|\mathcal{F}_{k-1} \right]-V(\btheta_{k-1})\right)1_{\{\btheta_{k-1}\not\in C\}}\leq -\tfrac{1}{2}\min\{1,\tfrac{1}{2}r\rho^*\}1_{\{\btheta_{k-1}\not\in C\}}.
\end{equation}
\end{proposition}

\begin{proof}
Suppose that $\btheta_{k-1}\not\in C$.  Lemma \ref{lem:hinge_loss_second_lemma} yields that 
\begin{equation}\label{eq:hinge_lemma_proposition_eq2}
     f(\rho_{k-1}\bmu)-f(\rho^*\bmu) \geq \tfrac{1}{2}r\rho^* \quad \text{ whenever } \vert \rho-\rho^* \vert \geq \tfrac{1}{2}\rho^*
\end{equation}
where constant $r$ is defined in \eqref{eq:constant_r_hinge_loss}. Moreover, from Lemma \ref{lem:hinge_high_noise_first_lemma}, we obtain that 
\begin{equation}\label{eq:hinge_lemma_proposition_eq1}
    f(\btheta_{k-1})-f(\rho_{k-1} \bmu)\geq 1 \quad \text{ whenever } \sigma \Vert \tilde{\btheta}_{k-1}\Vert \geq c \text{ and } \vert \rho-\rho^* \vert < \tfrac{1}{2}\rho^*.
\end{equation}
Moreover,
Combining \eqref{eq:hinge_lemma_proposition_eq1},   \eqref{eq:hinge_lemma_proposition_eq2} yields that 
\begin{equation}
    f(\btheta_{k-1})-f(\rho^*\bmu) \geq \min\{1,\tfrac{1}{2}r\rho^*\} \quad \text{ whenever } \btheta_{k-1} \not\in C.
\end{equation}
Lemma \eqref{lem:hinge_loss_high_noise_fundamental_lemma} and the bound on $\alpha$ in \eqref{bound_for_alpha_hinge_loss} along with the above displayed bound gives that 
\begin{equation}
    \bE\left[V(\btheta_k)|\mathcal{F}_{k-1} \right]-V(\btheta_{k-1}) \leq -\tfrac{1}{2}\min\{1,\tfrac{1}{2}r\rho^*\}.
\end{equation}
The proof is complete.
\end{proof}
\begin{proof}[Proof of Theorem \ref{thm:hinge_loss_high_noise}]
The target set $C$ defined in \eqref{target_set_for_hinge} is compact and thus there exists $b>0$ such that
\begin{equation}
    \left( \bE\left[V(\btheta_k)|\mathcal{F}_{k-1} \right]-V(\btheta_{k-1})\right)1_{\{\btheta_{k-1}\in C\}} \leq b1_{\{\btheta_{k-1}\in C\}}.
\end{equation}
Therefore, it holds that 
\begin{equation}\label{drift_for_hinge_loss}
    \bE\left[V(\btheta_k)|\mathcal{F}_{k-1} \right]-V(\btheta_{k-1}) \leq -\tfrac{1}{2}\min\{1,\tfrac{1}{2}r\rho^*\}1_{\{\btheta_{k-1}\not\in C\}}+b1_{\{\btheta_{k-1}\in C\}}.
\end{equation}
Furthermore, since $C$ is a compact set which does not contain $\bm{0}$, there exists a positive constant $\delta$ such that for any fixed $\btheta\in C$ it holds that 
\begin{equation}
    \delta:= \min \mathbb{P}_{\bxi \sim \mathcal{P}_*}\left(\bxi^T\btheta\geq 1 \right)>0.
\end{equation}
The result now follows from Appendix Lemma \ref{lem:drift_lemma_appendix} and Lemma \ref{lem:stopping_time_appendix}.
\end{proof}




==> temp.tex <==
In this section, we study the following optimization problem. 
\begin{align*}
  \min f(\btheta):= \bE_{(\bzeta,y) \sim \mathcal{P}} [\ell(\bzeta^T\btheta, y)] :=\bE_{(\bzeta,y) \sim \mathcal{P}} [ -y\bzeta^T\btheta + \log(1+ \exp(\bzeta^T\btheta))].
\end{align*}
We initialize with $\btheta_0=\bm{0}$. The SGD algorithm performs the following updates \begin{equation}
    \btheta_{k}=\btheta_{k-1}+ \frac{\alpha\bxi_{k-1}}{1+\exp\left(\bxi_{k-1}^T\btheta_k\right)}, \quad \bxi_{k-1} \stackrel{\text{i.i.d}}{\sim} N(\bmu,\sigma^2 I_d) \quad \forall k \geq 1.
\end{equation}
We state the main theorem of this section below. We defer the proof to the end of this subsection. 

\begin{theorem}\label{theorem_logistic}
Let $\btheta_0=\bm{0}$. The following are true.
\begin{enumerate}
    \item  Suppose that $\sigma \leq 0.16\Vert \bmu \Vert$ (low variance regime). The following then holds. 
\begin{equation}\begin{aligned} 
\bE[T]&\leq 4+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{29,584 \cdot (1+\alpha \Vert \bmu\Vert^2)^2}{\alpha \Vert \bmu\Vert^2}+15,224 \cdot \sigma^4\alpha^4\Vert \bmu\Vert^4\right)+\frac{14,792 \cdot (1+\alpha \Vert \bmu\Vert^2)^2}{\alpha\Vert\bmu\Vert^2}.
\end{aligned} \end{equation}  
\item Suppose that $0.16\Vert \bmu \Vert \leq \sigma$ (high variance regime).  It holds that $\bE[T]<+\infty$ provided $\alpha< \frac{\min\{1,B\}}{\Vert\bmu\Vert^2+d\sigma^2}$ where 
  \[
    B:=\tfrac{\Vert \bmu\Vert^4}{4\sigma^4\sqrt{\pi}}\exp\left(-\tfrac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \Phi^{c}\left( \tfrac{7\sqrt{2}\Vert \bmu \Vert}{\sigma}\right).
    \]
    In particular, the stopping criterion \eqref{eq: termination_test} terminates almost surely, provided that the step-size $\alpha$ is small enough. 
\end{enumerate}
  \end{theorem}
  
  \subsubsection{Low Variance Regime}\label{sec:low_log}
The main goal of this subsection is to give a proof of Theorem~\ref{theorem_logistic}.1. We restate it below.
\begin{manualtheorem}{2.1 }[]\label{thm.a}
Let $\btheta_0=\bm{0}$ and suppose that $\sigma \leq 0.16\Vert \bmu \Vert$. The following is then true. 
\begin{equation}\begin{aligned} 
\bE[T]&\leq 4+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{29,584 \cdot (1+\alpha \Vert \bmu\Vert^2)^2}{\alpha \Vert \bmu\Vert^2}+15,224 \cdot \sigma^4\alpha^4\Vert \bmu\Vert^4\right)+\frac{14,792 \cdot (1+\alpha \Vert \bmu\Vert^2)^2}{\alpha\Vert\bmu\Vert^2}.
\end{aligned} \end{equation}  
  \end{manualtheorem}
Recall that in the low variance regime (\textit{i.e.}, $\sigma \leq 0.16\Vert \bmu \Vert$), we define the target set by 
\begin{equation}\label{eq:C_low_proof}
    C=\{\btheta:\btheta^T\bmu\geq 1\}
\end{equation}
and the test function by 
\begin{equation}\label{eq:V_low_proof}
 V=\left(M-\bmu^T\btheta\right)^2
\end{equation}
where $M=86+86\alpha \Vert \bmu \Vert^2$. As we discussed earlier, our aim is to show that
\[
 \bE[\tau_m^C] \underset{\sim}{<} m.
\]
The following proposition bounds the expected value of the stopping time $\tau_1^C$ provided we initialize with $\btheta_0=\btheta$ such that $\bmu^T\btheta<1$.
\begin{proposition}\label{prp:low_et1} Fix a vector $\btheta \in \R^d$ such that $\bmu^T \btheta < 1$. Suppose that $\sigma\leq 0.16 \Vert \bmu \Vert$. Consider the set $C$ and the function $V$ defined in \eqref{eq:C_low_proof} and \eqref{eq:V_low_proof} respectively. Then the following bound holds
\begin{equation}
    \bE[\tau_1^{C}|\btheta_0=\btheta] \leq \frac{V(\btheta)}{\alpha \Vert \bmu \Vert^2}.
\end{equation}
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prp:low_et1}] For simplicity we write $\mathcal{F}_{-1}:=\sigma\left(\{\btheta_0=\btheta\} \right)$.  By expanding out the term, we get for any $k \ge 1$ the following
\begin{align} \label{eq: low_noise_blah_1}
    V(\btheta_{k})= V(\btheta_{k-1})-\frac{2\alpha \bmu^T\bxi_k(M-\bmu^T\btheta_{k-1})}{1+\exp(\bxi_k^T\btheta_{k-1})}+\frac{\alpha^2(\bmu^T\bxi_k)^2}{(1+\exp(\bxi_k^T\btheta_{k-1}))^2}.
\end{align}
We fix an integer $n \ge 1$ and write the quantity $\bmu^T\bxi_k=\Vert\bmu\Vert^2+\sigma\Vert \bmu\Vert \psi_k$ with $\psi_k \sim N(0,1)$. We have
\begin{align*}
 &\bE_{\bxi_k}\left[ \frac{\bmu^T\bxi_k}{1+\exp(\bxi_k^T\btheta_{k-1})}|\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
 & \qquad =\bE_{\bxi_k}\left[ \frac{\Vert\bmu\Vert^2}{1+\exp(\bxi_k^T\btheta_{k-1})}|\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}+\sigma \Vert \bmu\Vert\bE_{\bxi_k}\left[ \frac{\psi_k}{1+\exp(\bxi_k^T\btheta_{k-1})}|\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
 &  \qquad \geq \Vert \bmu \Vert^2 \bE_{\bxi_k}\left[ \frac{1}{1+\exp(\bxi_k^T\btheta_{k-1})}|\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}-\sigma \Vert \bmu\Vert\bE_{\psi_k}\left[ \vert \psi_k \vert\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
  &  \qquad \ge \Vert \bmu \Vert^2 \bE_{\bxi_k}\left[ \frac{1}{1+\exp(\bxi_k^T\btheta_{k-1})} \left ( 1_{\{\bmu^T \btheta_{k-1} \geq  \bxi_k^T \btheta_{k-1}\}} + 1_{\{\bmu^T \btheta_{k-1} < \bxi_k^T \btheta_{k-1}\}} \right ) |\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
  & \qquad \qquad \qquad -\sigma \Vert \bmu\Vert \sqrt{\frac{2}{\pi}}1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
 &  \qquad \geq \frac{\Vert \bmu\Vert^2}{1+\exp(\bmu^T\btheta_{k-1})}\bE_{\bxi_k}\left[ 1_{\{\bmu^T \btheta_{k-1} \geq  \bxi_k^T \btheta_{k-1}\}} |\mathcal{F}_{k-1} \right]1_{\{ \tau_1^{C}\wedge n \geq k\}}-\sigma \Vert \bmu\Vert \sqrt{\frac{2}{\pi}}1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
 &\qquad \geq \frac{\Vert \bmu\Vert^2}{2(1+e)}1_{\{ \tau_1^{C}\wedge n \geq k\}}-\sigma \Vert \bmu\Vert \sqrt{\frac{2}{\pi}}1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
 & \qquad \geq 0.006\Vert \bmu \Vert^2 1_{\{ \tau_1^{C}\wedge n \geq k\}}.
\end{align*}
Here the first inequality follows from $-\bE[X] \le \bE[|X|]$ and $1+ \exp(\bxi_k^T\btheta_{k-1}) \ge 1$, the second from ~\eqref{fact:norm_Gaussians}, and the second to last from the observation that for any $X$ normally distributed, $\bP(\bE[X] \ge X) = 1/2$ and $\bxi_k^T\btheta_{k-1} \sim N(\bmu^T\btheta_{k-1}, \sigma^2 \norm{\btheta_{k-1}}^2)$ and $\bmu^T\btheta_{k-1} < 1$ on the set $\tau_1^{C} \wedge n \ge k$. The last inequality uses the assumption $\sigma \le 0.16 \norm{\bmu}$. By taking the conditional expectations of \eqref{eq: low_noise_blah_1} combined with the above sequence of inequalities, we deduce the following bound
\begin{align*}
    &\bE\left[V(\btheta_{k})-V(\btheta_{k-1})|\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
    & \quad \qquad = \bE_{\bxi_k} \left [-\frac{2\alpha \bmu^T\bxi_k(M-\bmu^T\btheta_{k-1})}{1+\exp(\bxi_k^T\btheta_{k-1})} | \mathcal{F}_{k-1} \right] 1_{\{ \tau_1^{C}\wedge n \geq k\}} + \bE_{\bxi_k} \left [\frac{\alpha^2(\bmu^T\bxi_k)^2}{(1+\exp(\bxi_k^T\btheta_{k-1}))^2} | \mathcal{F}_{k-1} \right] 1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
    & \quad \qquad \leq -0.012(M-1)\alpha \Vert \bmu \Vert^21_{\{ \tau_1^{C}\wedge n \geq k\}}+ \alpha^2\Vert \bmu \Vert^2\left(\Vert \bmu\Vert^2+\sigma^2 \right)1_{\{ \tau_1^{C}\wedge n \geq k\}}\\
    & \quad \qquad = \alpha \Vert \bmu \Vert^2\left[ \alpha\left(\Vert \bmu \Vert^2+\sigma^2\right)-0.012(M-1)\right]1_{\{ \tau_1^{C}\wedge n \geq k\}}.
\end{align*}
Here the first inequality follows from $\bmu^T\btheta_{k-1} 1_{\{\tau_1^{C} \wedge n \ge k\}} \le 1_{\{\tau_1^{C}\wedge n \geq k\}}$ and upper bounding $\frac{(\bmu^T\bxi_k)^2}{(1+\exp(\bxi_k^T\btheta_{k-1}))^2}$ by $(\bmu^T\bxi_k)^2$ and then applying \eqref{fact:norm_Gaussians}.
A quick computation after plugging in the value of $M$ and the bound $\sigma\leq 0.16\Vert \bmu \Vert$ yields
\begin{equation} \label{eq: low_noise_blah_10}
  \bE\left[V(\btheta_{k})-V(\btheta_{k-1})|\mathcal{F}_{k-1}\right]1_{\{ \tau_1^{C}\wedge n \geq k\}} \leq -\alpha \Vert \bmu \Vert^21_{\{ \tau_1^{C}\wedge n \geq k\}}.
\end{equation}
Using Appendix Lemma \ref{lem:drift_lemma_appendix}, we obtain that $\bE[\tau_1^{C}\wedge n|\mathcal{F}_{-1}] \leq \frac{V(\btheta)}{\alpha \Vert \bmu \Vert^2}$. By monotone convergence theorem the result follows.
\end{proof}
We next upper bound $\bE[\tau_m^C]$ for $m\geq 1$ in the following proposition. 
\begin{proposition}\label{prp:low_etm}
Let $\btheta_0=\bm{0}$ and suppose that $\sigma\leq 0.16 \Vert \bmu \Vert$. Consider the set $C$ defined in \eqref{eq:C_low_proof}. Then the following bound holds for all $m \ge 1$
\begin{equation}
   \bE[\tau_m^C]\leq (m-1)\left(2+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{2M^2}{\alpha \Vert \bmu\Vert^2}+7,612 \cdot \sigma^4\alpha^4\Vert \bmu\Vert^4\right)\right)+\frac{M^2}{\alpha \Vert \bmu\Vert^2},
\end{equation}
where $M=86+86\alpha \Vert \bmu \Vert^2$.
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prp:low_etm}] 
First, it is clear when $m = 1$, the result holds by Proposition~\ref{prp:low_et1} with $\btheta_0 = \bm{0}$. We now assume that $\tau_{m-1}^{C}<\infty$ a.s. for some $m\geq 2$ and fix an integer $n \ge 1$. We decompose the space to yield the following bounds

 \begin{equation} \begin{aligned} \label{eq: low_noise_bound}
    \bE\left[(\tau_m^{C}-\tau_{m-1}^{C})\wedge n|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]&=\bE\left[((\tau_m^{C}-\tau_{m-1}^{C})\wedge n)|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]1_{\{\bmu^T\btheta_{\tau_{m-1}^{C}+1}\geq 1\}}\\
    &+\bE\left[((\tau_m^{C}-\tau_{m-1}^{C})\wedge n)|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]1_{\{\bmu^T\btheta_{\tau_{m-1}^{C}+1}<1\}}\\
    &\leq 1+ \bE\left[((\tau_m^{C}-\tau_{m-1}^{C})\wedge n)|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]1_{\{\bmu^T\btheta_{\tau_{m-1}^{C}+1}<1\}}\\
    &=1+\sum_{i=1}^{\infty}\bE\left[(\tau_m^{C}-\tau_{m-1}^{C})\wedge n|\mathcal{F}_{\tau_{m-1}^{C}+1}\right]1_{\{i-1\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}<i\}}\\
&\leq 2+\sum_{i=1}^{\infty}\bE\left[\tau_1^{C}\wedge n|\btheta_0=\btheta_{\tau_{m-1}^{C}+1}\right]1_{\{i-1\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}<i\}}.
\end{aligned} \end{equation}
Here the first inequality follows because $((\tau_m^{C}-\tau_{m-1}^{C})\wedge n) 1_{\{\bmu^T\btheta_{\tau_{m-1}^{C}+1} \ge 1\}} \le 1$ by definition of C and the last inequality by the strong Markov property. For each $i \ge 1$, we observe the bound
\begin{align}
  1-\bmu^T\btheta_{\tau_{m-1}^{C}+1} &=1-\bmu^T\btheta_{\tau_{m-1}^{C}}-\frac{\alpha \bmu^T\bxi_{{\tau_{m-1}^{C}}+1}}{1+\exp(\bxi_{{\tau_{m-1}^{C}}+1}^T\btheta_{\tau_{m-1}^{C}})}\nonumber\\
    &\leq -\frac{\alpha \bmu^T\bxi_{\tau_{m-1}^{C}+1}}{1+\exp(\bxi_{\tau_{m-1}^{C}+1}^T\btheta_{\tau_{m-1}^{C}})} \label{eq:i-1_calculus}\\
    & \leq -\alpha \bmu^T\bxi_{\tau_{m-1}^{C}+1},\nonumber
\end{align}
where the second inequality follows because $1-\bmu^T\btheta_{\tau_{m-1}^{C}} \le 0$ and the last inequality because $-\alpha \bmu^T \bxi_{\tau_{m-1}^{C}+1}$ is positive.  
By Proposition~\ref{prp:low_et1} and the above, we deduce 
\begin{equation} \begin{aligned}  \label{eq: low_noise_blah_3}
\bE\left[\tau_1^{C}\wedge n|\btheta_0=\btheta_{\tau_{m-1}^{C}+1}\right]1_{\{i-1\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}<i\}}&\leq  \frac{(M-\bmu^T\btheta_{\tau_{m-1}^{C}+1})^2}{\alpha \Vert \bmu \Vert^2}1_{\{i-1\leq 1-\bmu^T\btheta_{\tau_{m-1}^{C}+1}\leq i\}}\\&\leq  \frac{(M+i-1)^2}{\alpha \Vert \bmu\Vert^2}1_{\{ \bmu^T\bxi_{\tau_{m-1}^{C}+1}\leq \frac{1-i}{\alpha}\}}.
\end{aligned} \end{equation}
Finally we observe that 
\begin{equation} \begin{aligned} \label{eq: low_noise_blah_4}
    \bE\left[1_{\{ \bmu^T\bxi_{\tau_{m-1}^{C}+1}\leq \frac{1-i}{\alpha}\}} \right]&=\bE\left[\sum_{k=1}^{\infty}1_{\{ \bmu^T\bxi_{k+1}\leq \frac{1-i}{\alpha}\}}1_{\{\tau_{m-1}^{C}=k\}}\right]\\
&=\sum_{k=1}^{\infty}\bE\left[1_{\{ \bmu^T\bxi_{k+1}\leq \frac{1-i}{\alpha}\}}  \right]\bE\left[1_{\{\tau_{m-1}^{C}=k\}} \right]\\
    &= \Phi\left(\frac{\frac{1-i}{\alpha}-\Vert \bmu\Vert^2}{\sigma\Vert \bmu\Vert } \right)\sum_{k=1}^{\infty}\bE\left[1_{\{\tau_{m-1}^{C}=k\}} \right]\\
    &=\Phi\left(\frac{\frac{1-i}{\alpha}-\Vert \bmu\Vert^2}{\sigma\Vert \bmu\Vert } \right).
\end{aligned} \end{equation}
The first equality is by independence and the second equality because $\bmu^T \bxi_{k+1} \sim N(\norm{\bmu}^2, \sigma^2 \norm{\bmu}^2)$. Indeed, the same argument shows $\bxi_{\tau_{m-1}^{C}+1} \sim N(\bmu,\sigma^2I_d)$, see \cite[Theorem 4.3.1]{Durrett_probability_book}. By combining  \eqref{eq: low_noise_bound}, \eqref{eq: low_noise_blah_3}, and \eqref{eq: low_noise_blah_4}, we obtain the following
\begin{equation} \begin{aligned} \label{eq: low_noise_blah_5}
    \bE\left[(\tau_m^{C}-\tau_{m-1}^{C})\wedge n\right]&\leq 2+\sum_{i=1}^{\infty} \frac{(M+i-1)^2}{\alpha \Vert \bmu\Vert^2}\Phi\left(\frac{\frac{1-i}{\alpha}-\Vert \bmu\Vert^2}{\sigma\Vert \bmu\Vert } \right)\\&=2+\sum_{i=1}^{\infty} \frac{(M+i-1)^2}{\alpha \Vert \bmu\Vert^2}\Phi^{c}\left(\frac{\Vert \bmu\Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu\Vert } \right)\\&\le2+\frac{\sigma}{\Vert \bmu\Vert\sqrt{2\pi}}\sum_{i=1}^{\infty} \frac{(M+i-1)^2}{\alpha\Vert \bmu\Vert^2+i-1}\exp\left(-\frac{1}{2}\left(\frac{\Vert \bmu\Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu\Vert}\right)^2 \right),
\end{aligned} \end{equation}
where we used the inequality $\Phi^{c}(t)<\frac{1}{t\sqrt{2\pi}}\exp(-\frac{t^2}{2})$. We bound the sum by
\begin{equation}
\begin{aligned} \label{eq: low_noise_blah_6}
    \sum_{i=3}^{\infty} &\frac{(M+i-1)^2}{\alpha\Vert \bmu\Vert^2+i-1}\exp\left(-\frac{1}{2}\left(\frac{\Vert \bmu\Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu\Vert}\right)^2 \right)\\
    &\qquad = \sum_{i=3}^{\infty} \frac{(M+i-1)^2}{\alpha\Vert \bmu\Vert^2+i-1} \cdot \frac{4\sigma^4 \norm{\bmu}^2 \alpha^4}{(\alpha \norm{\bmu}^2 + i-1)^4} \cdot \frac{(\alpha \norm{\bmu}^2 + i-1)^4}{4\sigma^4 \norm{\bmu}^2 \alpha^4} \exp\left(-\frac{1}{2}\left(\frac{\Vert \bmu\Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu\Vert}\right)^2 \right)\\
    &\qquad \leq 4\alpha^4\sigma^4\Vert \bmu \Vert^4  \sum_{i=3}^{\infty}\frac{(M+i-1)^2}{(\alpha \Vert \bmu\Vert^2+i-1)^4}\\
    &\qquad \leq 29,584 \cdot \alpha^4\sigma^4\Vert \bmu\Vert^4 \sum_{i=3}^{\infty}\frac{1}{(i-1)^2} \\
    &\qquad \leq 29,584 \cdot \left ( \frac{\pi^2}{6}-1 \right ) \cdot \alpha^4\sigma^4\Vert \bmu\Vert^4\\ 
    & \qquad \leq 19,080 \cdot \alpha^4\sigma^4 \Vert \bmu\Vert^4.
\end{aligned} \end{equation}
Here the first inequality uses $x^2\leq e^x$ for all $x>0$ and $\alpha \norm{\bmu}^2 + i-1 \ge 1$ for all $i \ge 2$, the second uses that $\frac{M+i-1}{\alpha \Vert \bmu\Vert^2+i-1}\leq 86$ for all $i \ge 3$ and  $\frac{1}{\alpha \Vert \bmu\Vert^2+i-1}\leq \frac{1}{i-1}$ for $i\geq 2$. We also upper bound 

\begin{align} \label{eq: low_noise_blah_7}
  \sum_{i=1}^{2} \frac{(M+i-1)^2}{\alpha\Vert \bmu\Vert^2+i-1}\exp\left(-\frac{1}{2}\left(\frac{\Vert \bmu\Vert^2+\frac{i-1}{\alpha}}{\sigma\Vert \bmu\Vert}\right)^2 \right) &\leq \frac{M^2}{\alpha \Vert \bmu \Vert^2}+\frac{(M+1)^2}{\alpha \Vert \bmu \Vert^2+1} \le \frac{5M^2}{\alpha \norm{\bmu}^2},
\end{align}
where the first inequality we use $e^x \le 1$ for all $x<0$ and the second inequality because $\alpha \norm{\bmu}^2 + 1 \ge \alpha \norm{\bmu}^2$ and $M +1 \le 2M$. By combining \eqref{eq: low_noise_blah_5}, \eqref{eq: low_noise_blah_6}, and \eqref{eq: low_noise_blah_7}, we obtain 
\begin{align*}
   \bE\left[(\tau_m^{C}-\tau_{m-1}^{C})\wedge n\right]&\leq 2+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{2M^2}{\alpha \Vert \bmu\Vert^2}+7,612 \cdot \sigma^4\alpha^4\Vert \bmu\Vert^4\right).
   \end{align*}
Taking the limit as $n \to +\infty$, we observe that
\[\bE[\tau_m^C]\leq 2+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{2M^2}{\alpha \Vert \bmu\Vert^2}+7,612 \cdot \sigma^4\alpha^4\Vert \bmu\Vert^4\right)+\bE[\tau_{m-1}^{C}].
\]
We then iterate the above inequality yielding
\[ \bE[\tau_m^C] \le (m-1) \left ( 2+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{2M^2}{\alpha \Vert \bmu\Vert^2}+7,612 \cdot \sigma^4\alpha^4\Vert \bmu\Vert^4\right)  \right ) + \bE[\tau_1^{C}]. \]
The result follows after applying Proposition~\ref{prp:low_et1} with $\btheta_0 = \bm{0}$.
\end{proof}
We are now ready to prove Theorem~\ref{thm.a}.
\begin{proof}[Proof of Theorem
\ref{thm.a}]
In order to simplify the subsequent argument, we define the quantity, 
\[ M' := 2+\frac{\sigma}{\Vert \bmu\Vert}\left(\frac{2M^2}{\alpha \Vert \bmu\Vert^2}+7,612\sigma^4\alpha^4\Vert \bmu\Vert^4\right) \]
where $M = 86 + 86 \alpha \norm{\bmu}^2$, we see in Proposition~\ref{prp:low_etm}.  By Lemma \ref{lem:st_ETC},  $T_C<\infty$ a.s. and, therefore we have $\sum_{m=1}^{\infty}1_{\{T_C=\tau_m^{C}\}} = 1$ a.s. We next apply Proposition~\ref{prp:low_etm} with Lemma \ref{lem:st_ETC}. Note that $\delta:=\tfrac{1}{2}$ with the target set $C=\{\btheta:\bmu^T\btheta\geq 1 \}$ satisfy \eqref{eq:ST_delta}
\begin{align*}
\bE[T]&\leq \bE[T_C]=\sum_{m=1}^{\infty} \bE[\tau_C1_{\{T_C=\tau_m^{C}\}}]\leq \sum_{m=1}^{\infty}\frac{\bE[\tau_m^C]}{2^{m-1}} \le \sum_{m=1}^\infty \frac{(m-1)M' + \frac{M^2}{\alpha \norm{\bmu}^2} }{2^{m-1}} = 2M' + \frac{2M^2}{\alpha \norm{\bmu}^2}.
\end{align*}
The result follows after plugging in the value of $M = 86 + 86 \alpha \norm{\bmu}^2$.
\end{proof}

\subsubsection{High Variance Regime}\label{sec:high_logistic}
The main goal of this subsection is to give a proof of Theorem~\ref{theorem_logistic}.2. We restate it below.
\begin{manualtheorem}{2.2}[]\label{thm.b}
Let $\btheta_0=\bm{0}$ and suppose that $ 0.16\Vert \bmu \Vert \leq \sigma$. Then it holds that $\bE[T]<+\infty$ provided the step-size $\alpha$ satisfies  
\begin{equation}\label{eq:high_alpha}
\alpha < \tfrac{\min\{1,B\}}{\Vert \bmu \Vert^2+d\sigma^2} 
\end{equation}
where the constant $B$ is defined by 
\begin{equation}
B:=\tfrac{\Vert \bmu\Vert^4}{4\sigma^4\sqrt{\pi}}\exp\left(-\tfrac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \Phi^{c}\left( \tfrac{7\sqrt{2}\Vert \bmu \Vert}{\sigma}\right).
\end{equation}
  \end{manualtheorem}
The proof is deferred to the end of this subsection. We first need some preliminaries. Throughout this subsection, the following notation is used
\[
 \btheta = \rho\bmu+ \bm{\tilde{\theta}} \text{ where } \bmu^T \bm{\tilde{\theta}} = 0.
\]
We also express $\btheta_k=\rho_k\bmu+\tilde{\btheta}_k$, etc.  Recall that in the high variance regime (\textit{i.e.}, $0.16\Vert \bmu \Vert\leq \sigma$), we define the target set by 
\begin{equation}\label{eq:C_high_proof_1}
     C=\left\{\btheta: \vert \rho\sigma^2-2\vert < 1 \text{ and } \sigma \Vert \tilde{\btheta} \Vert \leq 3404.46 \right\}.`
\end{equation}
We first establish \eqref{eq:ST_delta}.

\begin{lemma}\label{lem: high_noise_delta}
Consider the set defined in \eqref{eq:C_high_proof_1}. Fix $\btheta\in {C}$ and let $\hat{\bxi} \sim N(\bmu,\sigma^2 I_d)$. The following bound holds.
\begin{equation}\label{eq:deltaP}
    \bP_{\hat{\bxi}}\left(\btheta^T\hat{\bxi}\geq 1\right)\geq \Phi\left(\frac{-\sigma}{\Vert \bmu \Vert}\right).
\end{equation}
\end{lemma}

\begin{proof}
It is easy to verify that $\bP_{\hat{\bxi}}\left(\btheta^T\hat{\bxi}\geq 1\right)=\Phi\left(\frac{\btheta^T\bmu-1}{\sigma \Vert \btheta\Vert} \right)$. We are interested in lower bounding the term $\frac{\btheta^T\bmu-1}{\sigma \Vert \btheta\Vert}$ independent of $\btheta$. 
%We have 
%\begin{align*}
 %   \sigma \Vert \btheta\Vert &\leq \vert \rho \sigma\vert \Vert \bmu\Vert+ \sigma\Vert \tilde{\btheta}\Vert\\&\leq \vert \rho\sigma^2\vert\frac{\Vert \bmu\Vert}{\sigma}+\sigma\Vert \tilde{\btheta}\Vert\\&\leq \frac{3}{s}+24s'.
%\end{align*}
As $\btheta \in {C}$, we have $\vert \rho\sigma^2-2\vert < 1$ which yields $\rho \geq \frac{1}{\sigma^2}$. Combining this with $\Vert \btheta \Vert^2 = \| \rho \bmu + \tilde{\btheta} \|^2 \geq \rho^2\Vert \bmu \Vert^2$, we obtain that $\sigma \Vert \btheta \Vert\geq \frac{\Vert \bmu \Vert}{\sigma}$. This gives
\begin{equation}
     \frac{\btheta^T\bmu-1}{\sigma \Vert \btheta\Vert} = \frac{(\rho \bmu + \tilde{\btheta})^T\bmu-1}{\sigma \norm{\btheta}} \geq \frac{-1}{\sigma \Vert \btheta\Vert}\geq  \frac{-\sigma}{\Vert \bmu \Vert}.
\end{equation}
Here the first inequality follows from $\rho>0$ and the second inequality from $\sigma \Vert \btheta \Vert\geq \frac{\Vert \bmu \Vert}{\sigma}$. The proof is complete after noting that $\Phi$ is an increasing function.
\end{proof}
We need the following technical lemma below. The proof is deferred to Appendix Sec. ???. 

\begin{lemma}\label{lem:high_tech_not_appendix}
Consider the following optimization problem 
\[
\min f(\btheta):=\bE_{(\bxi,y)\sim \mathcal{P}_*}\left[\ell(\bxi^T\btheta,y)\right].
\]
where $\ell$ is a convex function. The sequences $\{\bm{\theta}_k, \bm{\xi}_k \}_{k = 0}^\infty$ generated by Algorithm~\ref{alg:SGD_termination} satisfy for any $\bm{\theta} \in \R^d$, the following
    \begin{equation} \label{eq:tech_lemma_inside}
       f(\bm{\theta}_{k-1})-f(\bm{\theta})\leq \frac{1}{2\alpha}\left(\Vert  \bm{\theta}_{k-1}-\bm{\theta} \Vert^2-\bE\left[\Vert \bm{\theta}_{k}-\bm{\theta} \Vert^2\, |\mathcal{F}_{k-1}\right] \right)+\bE[\Vert\nabla_{\btheta}\ell\left( \bxi_k^T\btheta\right)\Vert^2 \, | \, \mathcal{F}_{k-1}],
    \end{equation}
    for all $k\geq 1$ where $f$ is defined in \eqref{optimization_problem} and the filtration $\{\mathcal{F}_k\}_{k=0}^{+\infty}$ in \eqref{eq:sigma}.
\end{lemma}
\begin{remark}
Note that in \eqref{eq:tech_lemma_inside}, we are not assuming that $\ell$ is differentiable. We have two choices for the $\ell$ function: logistic loss and hinge loss. Nevertheless, hinge loss is not differentiable, since for any $\btheta$ w.p. 1 $\bxi_k^T\btheta\neq 1$, we conclude that $\ell(\bxi_k^T\btheta)$ as a function of $\bxi_k$ is almost everywhere differentiable.
\end{remark}



Let $\btheta$ be $\btheta^*$  in Lemma~\ref{lem:high_tech_not_appendix} and write 
\begin{equation}\label{eq:high_ftheta_ktheta}
    f(\btheta_{k-1})-f(\btheta^*)=f(\btheta_{k-1})-f(\rho\bmu)+f(\rho\bmu)-f(\btheta^*).
\end{equation}
In Lemmas~\ref{lem: logistic_case_2} and \ref{lem: logistic_case_1} below, we will show that both terms $f(\btheta_{k-1})-f(\rho \bmu)$ and $f(\rho\bmu)-f(\btheta^*)$ are non-negative. Moreover, we will establish that whenever $\btheta_{k-1} \not\in C$, either the first or second term can be lower bounded by some positive constant.  We first lower bound $f(\btheta_{k-1})-f(\rho \bmu)$.  Let us recall that $\btheta=\rho \bmu+\tilde{\btheta}$ where $\hat{\btheta}^T\bmu=0$.
\begin{lemma} \label{lem: logistic_case_2} Fix a vector $\btheta \in \R^d$ and let $\bxi \sim N(\bmu,\sigma^2I_d)$. Provided that $\sigma \Vert \tilde{\btheta}\Vert\geq 4\log(\sqrt{2}+1)$, the following holds
\begin{equation}\label{eq:high_lem_sigmatheta}
    \bE_{\bxi} \left[\log\left( \frac{1+\exp(-\btheta^T\bxi)}{1+\exp(-\rho \bmu^T\bxi)}\right)\right] \geq \max\left\{\left ( \tfrac{1}{2} \log(2) + \tfrac{\sigma \Vert \tilde{\btheta}\Vert}{8} \right )\Phi^c(1)-\left | \frac{\rho}{4}\right | \left(\Vert \bmu\Vert^2+\sigma \Vert \bmu \Vert \sqrt{\frac{2}{\pi}} \right)
    ,0\right\}.
\end{equation}

% \max\left\{0.085\sigma \Vert \tilde{\btheta}\Vert+0.029-\left | \frac{\rho}{4}\right | \left(\Vert \bmu\Vert^2+\sigma \Vert \bmu \Vert \sqrt{\frac{2}{\pi}} \right)
%     ,0\right\}.

\end{lemma}
\begin{proof} The two normal random variables, $\bm{\tilde{\theta}}^T\bm{\xi} \sim N(0,\sigma^2\Vert \bm{\tilde{\theta}} \Vert^2)$ and $\bmu^T\bxi \sim N(\Vert \bmu \Vert^2,\sigma^2\Vert \bmu \Vert^2)$, are independent by \eqref{eqn:fact_independence}. Since we have $\bE_{\bxi}[\log(\exp(-\bm{\tilde{\theta}}^T\bxi))]=\bE_{\bxi}[\log(\exp(\bm{\tilde{\theta}}^T\bxi))]=0$, it holds
\begin{align*}
    \bE_{\bxi} \left[ \log\left (1+\exp(-\btheta^T\bxi)\right)\right] &= \bE_{\bxi} \left[\log \left(1 + \exp(-\tilde{\btheta}^T\bxi) \exp(-\rho \bmu^T\bxi) \right ) \right ]\\
    &=\bE_{\bxi} \left[ \log\left (\exp(\bm{\tilde{\theta}}^T\bxi)+\exp(-\rho \bmu^T\bxi)\right)\right]\\
    &=\bE_{\bxi} \left[ \log\left (\exp(-\bm{\tilde{\theta}}^T\bxi)+\exp(-\rho \bmu^T\bxi)\right)\right],
\end{align*}
where the last equality is true because $\bm{\tilde{\theta}}^T\bxi \sim -\bm{\tilde{\theta}}^T\bxi$. Therefore we obtain
\begin{align*}
  \bE_{\bxi} &\left[ \log\left (1+\exp(-\btheta^T\bxi)\right)\right]\\
  & \qquad \qquad= \frac{1}{2} \bE_{\bxi} \left[ \log\left (\exp(\bm{\tilde{\theta}}^T\bxi)+\exp(-\rho \bmu^T\bxi)\right)\right] + \frac{1}{2}\bE_{\bxi} \left[ \log\left (\exp(-\bm{\tilde{\theta}}^T\bxi)+\exp(-\rho \bmu^T\bxi)\right)\right] \\
  & \qquad \qquad= \frac{1}{2} \bE_{\bxi} \left[ \log\left ( (\exp(\bm{\tilde{\theta}}^T\bxi)+\exp(-\rho \bmu^T\bxi))(\exp(-\bm{\tilde{\theta}}^T\bxi)+\exp(-\rho \bmu^T\bxi)) \right)\right]\\ 
  &\qquad \qquad=\frac{1}{2}\bE_{\bxi} \left[\log\left(1+\exp(-\bm{\tilde{\theta}}^T\bxi-\rho \bmu^T\bxi)+\exp(\bm{\tilde{\theta}}^T\bxi-\rho \bmu^T\bxi)+\exp(-2\rho \bmu^T\bxi)\right) \right].
  \end{align*}
By the equality $\exp(\bm{\tilde{\theta}}^T\bxi)+\exp(-\bm{\tilde{\theta}}^T\bxi)= 2+4\sinh^2(\tfrac{\tilde{\btheta}^T\bxi}{2})$, we have
\begin{align*}
   \bE_{\bxi} &\left[ \log\left (1+\exp(-\btheta^T\bxi)\right)\right]\\
    & \qquad \qquad \qquad =\frac{1}{2}\bE_{\bxi} \left[\log\left(1+2\exp(-\rho \bmu^T\bxi)+\exp(-2\rho \bmu^T\bxi)+4\sinh^2(\tfrac{\tilde{\btheta}^T\bxi}{2})\exp(-\rho \bmu^T\bxi)\right) \right].
\end{align*}
Therefore, we have
\begin{equation} \begin{aligned} \label{eqn: high_noise_blah_20}
     2\bE_{\bxi}\left[\log\left( \frac{1+\exp(-\btheta^T\bxi)}{1+\exp(-\rho \bmu^T\bxi)}\right)\right]&=2\bE_{\bxi}\left[\log(1+\exp(-\btheta^T\bxi))\right]-\bE_{\bxi}\left[\log\left(1+\exp(-\rho \bmu^T\bxi)\right)^2\right]\\
     \qquad \qquad &= \bE_{\bxi}\left[\log \left ( 1 +  \frac{4\sinh^2(\frac{\tilde{\btheta}^T\bxi}{2})\exp(-\rho \bmu^T\bxi)}{(1+ \exp(-\rho \bmu^T\bxi))^2} \right ) \right] \ge 0.
     \end{aligned} \end{equation}
     Thus it remains to establish the other lower bound in \eqref{eq:high_lem_sigmatheta}. First, we note the following $1+ \exp(-\rho \bmu^T\bxi) = 2 \exp( -\tfrac{\rho \bmu^T\bxi}{2}) \cosh(\tfrac{\rho \bmu^T\bxi}{2})$. Let the constant $r > 0$ and consider the set $\{\bxi: |\btheta^T\bxi| > r\}$. Applying the inequality $x^2+y^2\geq 2\vert xy \vert$ and \eqref{eqn: high_noise_blah_20}, we obtain that 
     \begin{align}
   2\bE_{\bxi}\left[\log\left( \frac{1+\exp(-\btheta^T\bxi)}{1+\exp(-\rho \bmu^T\bxi)}\right)\right]  & = \bE_{\bxi}\left[\log\left(1 + \frac{4\sinh^2(\frac{\tilde{\btheta}^T\bxi}{2})\exp(-\rho \bmu^T\bxi)}{(1+ \exp(-\rho \bmu^T\bxi))^2}\right) \right] \nonumber \\ 
     &= \bE_{\bxi}\left[\log\left(1+\frac{\sinh^2(\frac{\tilde{\btheta}^T\bxi}{2})}{\cosh^2(\frac{\rho}{2}\bmu^T\bxi)} \right) \right] \nonumber \\ 
     &\geq \bE_{\bxi}\left[\log\left(1+\frac{\sinh^2(\frac{\tilde{\btheta}^T\bxi}{2})}{\cosh^2(\frac{\rho}{2}\bmu^T\bxi)} \right) 1_{\{\bxi:\vert \tilde{\btheta}^T\bxi\vert \geq r\}}\right] \label{eq:high_noise_blah_21}
     \\
     &\geq \bE_{\bxi}\left[\left(\log2+\log\left( \frac{\vert\sinh(\frac{\tilde{\btheta}^T\bxi}{2})\vert}{\cosh(\frac{\rho}{2}\bmu^T\bxi)}\right) \right)1_{\{\bxi:\vert \tilde{\btheta}^T\bxi\vert \geq r\}}\right] \nonumber.
    \end{align}
Here  \eqref{eq:high_noise_blah_21} follows from $\log\left(1+\frac{\sinh^2(\frac{\tilde{\btheta}^T\bxi}{2})}{\cosh^2(\frac{\rho}{2}\bmu^T\bxi)} \right)$ is always positive. From \eqref{eq:fact_affine}, we have $\bmu^T\bxi \sim N(\Vert \bmu \Vert^2,\sigma^2\Vert \bmu \Vert^2)$ and $\tilde{\btheta}^T\bxi \sim N(0,\sigma^2\Vert \tilde{\btheta} \Vert^2)$. Thus, we write $\tilde{\btheta}^T\bxi = \sigma \| \tilde{\btheta} \| \psi$ where $\psi \sim N(0,1)$. Moreover, we have that $-\log\left(\cosh(\frac{\rho}{2}\bmu^T\bxi)\right)1_{\{\vert \tilde{\btheta}^T\bxi\vert \geq r\}} \geq -\log\left(\cosh(\frac{\rho}{2}\bmu^T\bxi)\right) $ since $\cosh(\frac{\rho}{2}\bmu^T\bxi)\geq 1$ always holds. Using the inequality $\log\cosh(x)\leq \vert x\vert$ for all $x$, the following bound holds
     \begin{equation} \begin{aligned} \label{eq: high_noise_22}
       &\bE_{\bxi}\left[\log\left( \frac{1+\exp(-\btheta^T\bxi)}{1+\exp(-\rho \bmu^T\bxi)}\right)\right]\\
       & \quad \ge \tfrac{1}{2} \log(2) \cdot \bE_{\psi}\left[1_{\{\vert \psi\vert \geq \frac{r}{\sigma \Vert\tilde{\btheta}\Vert}\}}\right] + \tfrac{1}{2} \bE_{\psi}\left[\log\left\vert\sinh(\tfrac{\sigma\Vert \tilde{\btheta}\Vert\psi}{2})\right\vert1_{\{\vert \psi\vert \geq \frac{r}{\sigma \Vert\tilde{\btheta}\Vert}\}}\right] - \tfrac{1}{2}\bE_{\bxi} \left [ \log( \cosh(\tfrac{\rho}{2} \bmu^T\bxi)) \right ]\\
       & \quad \ge \tfrac{1}{2} \log(2) \cdot \bE_{\psi}\left[1_{\{\vert \psi\vert \geq \frac{r}{\sigma \Vert\tilde{\btheta}\Vert}\}}\right] + \tfrac{1}{2} \bE_{\psi}\left[\log\left\vert\sinh(\tfrac{\sigma\Vert \tilde{\btheta}\Vert\psi}{2})\right\vert1_{\{\vert \psi\vert \geq \frac{r}{\sigma \Vert\tilde{\btheta}\Vert}\}}\right] - \tfrac{1}{2} \bE_{\bxi} \left [ | \tfrac{\rho}{2} \bmu^T\bxi | \right ]\\
       &\quad\geq \tfrac{1}{2} \log(2) \cdot \bE_{\psi}\left[1_{\{\vert \psi\vert \geq \frac{r}{\sigma \Vert\tilde{\btheta}\Vert}\}}\right] + \tfrac{1}{2} \bE_{\psi}\left[\log\left\vert\sinh(\tfrac{\sigma\Vert \tilde{\btheta}\Vert\psi}{2})\right\vert1_{\{\vert \psi\vert \geq \frac{r}{\sigma \Vert\tilde{\btheta}\Vert}\}}\right]-\left | \frac{\rho}{4}\right | \left(\Vert \bmu\Vert^2+\sigma \Vert \bmu \Vert \sqrt{\frac{2}{\pi}} \right), 
    \end{aligned} \end{equation}
where the last inequality uses \eqref{fact:norm_Gaussians}. Using the inequality $\vert \sinh(x) \vert \geq \exp(\frac{\vert x\vert}{2})$ for $\vert x \vert \geq 2\log(\sqrt{2}+1)$, letting $r=4\log(\sqrt{2}+1)$, we obtain 
\begin{align}
   \tfrac{1}{2} \log(2) \cdot \bE_{\psi} \big [ 1_{\{|\psi| \ge \frac{4 \log( \sqrt{2}+ 1)\}}{\sigma \norm{\tilde{\btheta}} }} \big ] &+ \tfrac{1}{2}\bE_\psi\left[\log\left\vert\sinh(\tfrac{\sigma\Vert \tilde{\btheta}\Vert\psi}{2})\right\vert1_{\{|\psi| \geq \frac{4\log(\sqrt{2}+1)}{\sigma \Vert \tilde{\btheta}\Vert}\}}\right]\nonumber\\
   &\geq \tfrac{1}{2} \log(2) \cdot \bE_{\psi} \big [ 1_{\{|\psi| \ge \frac{4 \log( \sqrt{2}+ 1)}{\sigma \norm{\tilde{\btheta}} } \}} \big ] +  \tfrac{1}{2}\bE_\psi\left[\left\vert\tfrac{\sigma \Vert \tilde{\btheta}\Vert \psi}{4} \right\vert1_{\{|\psi| \geq \frac{4\log(\sqrt{2}+1)}{\sigma \Vert \tilde{\btheta}\Vert}\}}\right]\nonumber\\
    &\geq \tfrac{1}{2} \log(2) \cdot \bE_{\psi}[1_{\{\vert\psi\vert \ge 1\}}] + \tfrac{1}{2} \bE_\psi\left[\left\vert\tfrac{\sigma \Vert \tilde{\btheta}\Vert \psi}{4} \right\vert1_{\vert\psi\vert \geq 1\}}\right] \label{eq:high_noise_blah_111} \\\nonumber
    &\geq \left ( \tfrac{1}{2} \log(2) + \frac{\sigma \Vert \tilde{\btheta}\Vert}{8} \right )\Phi^c(1).
    % &\geq 0.085 \sigma \Vert \tilde{\btheta} \Vert.
\end{align}
Here \eqref{eq:high_noise_blah_111} follows from $1\geq \frac{4\log(\sqrt{2}+1)}{\sigma \Vert \tilde{\btheta}\Vert}
$. By combining the above inequality with \eqref{eq: high_noise_22}, the desired result holds. 
\end{proof}
We now turn to lower bound the second summand in the right-hand side of \eqref{eq:high_ftheta_ktheta}, namely $f(\rho \bmu)-f(\bm{\theta^*})$.
\begin{lemma} \label{lem: logistic_case_1}
Provided that $\vert \rho\sigma^2-2 \vert> 1$, the following estimate holds
\begin{equation}\label{eq:high_lemhrho}
    f(\rho \bmu)-f(\bm{\theta^*}) \geq \frac{\Vert \bmu\Vert^4}{4\sigma^4\sqrt{\pi}}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \Phi^{c}\left( \frac{7\sqrt{2}\Vert \bmu \Vert}{\sigma}\right).
\end{equation}

\end{lemma}
\begin{proof} Define the function
\[
    g(\rho):=\bE_{\bxi}\left[\log\left(1+\exp(-\rho \bmu^T\bxi)\right) \right], \quad \bxi \sim N(\bmu,\sigma^2I_d).
\]
By Lemma~\ref{lem:minimizer_logistic}, we know that $g$ is a convex function with a unique minimizer at $\rho^*:=\frac{2}{\sigma^2}$. Observe that $f(\rho \bmu)-f(\btheta^*) = g(\rho)-g(\rho^*)$; hence in order to prove \eqref{eq:high_lemhrho}, we instead aim to bound this difference in the function $g$. From \eqref{eq:fact_affine}, we have $\bmu^T\bxi \sim N(\Vert \bmu \Vert^2,\sigma^2\Vert \bmu \Vert^2)$. It thus holds
\[
 4g''(\rho)=\bE\left(\frac{(\bmu^T\bxi)^2}{\cosh(\frac{\rho}{2} \bmu^T\bxi)^2} \right)=\frac{1}{\sigma\Vert \bmu\Vert\sqrt{2\pi }}\int_{-\infty}^{\infty}\frac{z^2}{\cosh^2(\frac{\rho z}{2})}\exp\left(-\frac{(z-\Vert \bmu \Vert^2)^2}{2\sigma^2\Vert \bmu \Vert^2}\right)dz.
\]
Upper bounding $\cosh^2(\frac{\rho z}{2})$ by $\exp(\vert \rho z\vert)$, we next obtain
\begin{align*}
    4g''(\rho)&\geq \frac{1}{\sigma\Vert \bmu\Vert\sqrt{2\pi}} \int_{-\infty}^{\infty} z^2\exp\left(-\vert \rho z \vert \right)\exp\left(-\frac{(z-\Vert \bmu \Vert^2)^2}{2\sigma^2\Vert \bmu\Vert^2}\right)dz & \\ &=\frac{1}{\sigma\Vert \bmu\Vert\sqrt{2\pi }} \int_{-\infty}^{\infty} z^2\exp\left(-\frac{(z-\Vert \bmu \Vert^2)^2+2\sigma^2\Vert \bmu\Vert^2\vert\rho z\vert}{2\sigma^2\Vert \bmu\Vert^2}\right)dz  ,&\\
    &=\frac{1}{\sigma\Vert \bmu\Vert\sqrt{2\pi }}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2} \right) \int_{-\infty}^{\infty} z^2\exp\left(-\frac{z^2-2\Vert \bmu \Vert^2 z+2\sigma^2\Vert \bmu\Vert^2\vert\rho z\vert}{2\sigma^2\Vert \bmu\Vert^2}\right)dz
\end{align*}
One can easily verify that whenever $\vert z \vert \geq 2\Vert \bmu \Vert^2 +2\sigma^2\Vert \bmu\Vert^2 \vert \rho \vert$ yields
\begin{equation*}
    \exp\left(-\frac{z^2-2\Vert \bmu \Vert^2 z+2\sigma^2\Vert \bmu\Vert^2\vert\rho z\vert}{2\sigma^2\Vert \bmu\Vert^2}\right) \geq \exp\left(-\frac{z^2}{\sigma^2\Vert \bmu\Vert^2} \right).
\end{equation*}
Therefore, we have
\begin{equation*}
    4g''(\rho) \geq \frac{2}{\sigma\Vert \bmu\Vert\sqrt{2\pi }}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2} \right) \int_{2\Vert \bmu \Vert^2 +2\sigma^2\Vert \bmu\Vert^2 \vert \rho \vert}^{\infty} z^2\exp\left(-\frac{z^2}{\sigma^2\Vert \bmu\Vert^2} \right)dz.
\end{equation*}
%Let the constant $\rho^* := \frac{2}{\sigma^2}$.
The change of variables $z \mapsto \frac{\sigma\Vert\bmu\Vert}{\sqrt{2}} z$ yields 
\begin{align*}
   g''(\rho) &\geq \frac{\sigma^2\Vert \bmu\Vert^2}{8\sqrt{\pi}}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \int_{ 2\sqrt{2}(1+2\vert \frac{\rho}{\rho^*}\vert)\frac{\Vert \bmu \Vert}{\sigma}}^{\infty} z^2\exp\left(-\frac{z^2}{2}\right)dz\\
%   &\geq \frac{\sigma^2\Vert \bmu\Vert^2}{8\sqrt{\pi}}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \int_{ \frac{r_\rho\Vert \bmu \Vert}{\sigma}}^{\infty} z^2\exp\left(-\frac{z^2}{2}\right)dz \\
   &\geq \frac{\Vert \bmu \Vert^4}{\sqrt{\pi}}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \int_{ 2\sqrt{2}(1+2\vert \frac{\rho}{\rho^*}\vert)\frac{\Vert \bmu \Vert}{\sigma}}^{\infty} \exp\left(-\frac{z^2}{2}\right)dz,
 \end{align*}
where the last inequality holds because $z^2 \ge \frac{8\norm{\bmu}^2}{\sigma^2}$ on the interval $[2\sqrt{2}(1+2 |\tfrac{\rho}{\rho^*}|) \tfrac{\norm{\bmu}}{\sigma}, \infty)$. Let $r(\rho) :=2\sqrt{2}(1+2\vert \frac{\rho}{\rho^*}\vert)$. 
 Continuing, we get \begin{equation*}
     g''(\rho) \geq\frac{\Vert \bmu \Vert^4}{\sqrt{\pi}}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \Phi^{c}\left( \frac{r(\rho)\Vert \bmu \Vert}{\sigma}\right).
 \end{equation*}
 The proof now follows from Lemma \ref{lem:high_tech_not_appendix}.
 
\end{proof}
Let us recall that we define the target set $C$ by 
\begin{equation}\label{eq:C_high_proof}
   C=\left\{\btheta: \vert \rho\sigma^2-2\vert < 1 \text{ and } \sigma \Vert \tilde{\btheta} \Vert \leq c \right\},
\end{equation}
where the constant $c$ is \begin{equation}\label{eq:c_high_proof}
    c=8\left(\frac{\tfrac{3}{2}\left(\frac{1}{0.16^2}+\sqrt{\frac{2}{\pi}}\frac{1}{0.16} \right)+1}{\Phi^c(1)}-\tfrac{1}{2}\log(2)\right) \approx 3404.46.
\end{equation}
The next proposition establishes the desired bound $\bE[\tau_m^C] \underset{\sim}{<} m.$ Note that the set $C$ is compact. This implies that the value of the test function at the next iteration increases, in expectation, by at most a fixed constant whenever the current iterate is inside $C$. This facilitates establishing bounds for $\bE[\tau_C^m]$ as we will in the proof of following proposition.
\begin{proposition}\label{prp:high_V} Let $\btheta_0=\bm{0}$ and suppose that $0.16\Vert \bmu \Vert \leq\sigma$. Consider the set $C$ defined in \eqref{eq:C_high_proof}.
%  Define the following test function on $\R^d$
% \[
% V(\btheta)=\frac{\Vert \btheta-\btheta^*\Vert^2}{\alpha\min\{1,B\}},
% \]
% where $B$ is defined by $B:=\frac{\Vert \bmu\Vert^4}{4\sigma^4\sqrt{\pi}}\exp\left(-\frac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \Phi^{c}\left( \frac{7\sqrt{2}\Vert \bmu \Vert}{\sigma}\right)$ and 
Let the step-size $\alpha > 0$ satisfy
\begin{equation}\label{eq:high_noise_alpha_assumption}
\alpha < \frac{\min\{1,B\}}{\Vert \bmu \Vert^2+d\sigma^2},
\end{equation}
where the constant $B$ is 
\begin{equation}
B:=\tfrac{\Vert \bmu\Vert^4}{4\sigma^4\sqrt{\pi}}\exp\left(-\tfrac{\Vert \bmu \Vert^2}{2\sigma^2}\right) \Phi^{c}\left( \tfrac{7\sqrt{2}\Vert \bmu \Vert}{\sigma}\right).
\end{equation}
Then the following is true
\begin{equation}\label{eq:high_Tm}
    \bE\left[\tau_m^{C}\right]\leq
    \frac{\Vert \bmu \Vert^2}{4\alpha\sigma^4\min\{ 1,B\}}+(m-1)\left(2+\frac{\Vert \bmu \Vert^2+c\sigma^2}{\alpha \sigma^4\min\{1,B\}}\right).
\end{equation}
\end{proposition}
\begin{proof}[Proof of Proposition \ref{prp:high_V}] To simplify the subsequent argument, we define the test function $\overline{V}$ by
\[
\overline{V}(\btheta)=\frac{\Vert \btheta-\btheta^*\Vert^2}{\alpha\min\{1,B\}}.
\]
We first establish the drift equation \eqref{eq:st_VoutC} for the test function $\overline{V}$ and the target set \eqref{eq:C_high_proof}. To do so, we first show that 
\begin{equation}\label{eq:high_thetak}
 f(\btheta_{k-1})-f(\btheta^*) \geq \min\{1,B\}1_{\{\btheta_{k-1}\not\in {C}\}}.
\end{equation}
% Recall that the set ${C}$ is defined by 
% \begin{equation*}
% {C}=\left\{\btheta: \vert \rho\sigma^2-2\vert < 1 \text{ and } \sigma \Vert \tilde{\btheta} \Vert \leq 385.593 \right\}.
% \end{equation*}
Clearly \eqref{eq:high_thetak} holds when $\btheta_{k-1}\in {C}$ so suppose that $\btheta_{k-1}\not\in {C}$. Therefore, either we have $\vert\rho_{k-1}\sigma^2-2\vert>1$ or $\sigma \Vert \tilde{\btheta}_{k-1}\Vert \geq c$. If $\vert\rho_{k-1}\sigma^2-2\vert>1$, then Lemma \ref{lem: logistic_case_1} yields that $ f(\rho_{k-1}\bmu)-f(\btheta^*)\geq B$. Then we write that 
\begin{equation}
     f(\btheta_{k-1})-f(\btheta^*)=\underbrace{f(\btheta_{k-1})-f(\rho_{k-1}\bmu)}_{\geq 0 \text{ by Lemma~\ref{lem: logistic_case_2} }}+f(\rho_{k-1}\bmu)-f(\btheta^*) \geq B,
\end{equation}
establishing \eqref{eq:high_thetak}. So assume $\vert \rho_{k-1} \sigma^2-2\vert<1$ and hence $\sigma \Vert \tilde{\btheta}_{k-1}\Vert \geq c$. We obtain that
\begin{align}
     \bE_{\bxi_k} \left[\log\left( \frac{1+\exp(-\btheta_{k-1}^T\bxi_k)}{1+\exp(-\rho_{k-1} \bmu^T\bxi_k)}\right)\right]&\geq \left ( \tfrac{1}{2} \log(2) + \tfrac{\sigma \Vert \tilde{\btheta}\Vert}{8} \right )\Phi^c(1)-\left | \frac{\rho_{k-1}}{4}\right | \left(\Vert \bmu\Vert^2+\sigma \Vert \bmu \Vert \sqrt{\frac{2}{\pi}} \right)\nonumber\\&\geq \left ( \tfrac{1}{2} \log(2) + \tfrac{\sigma \Vert \tilde{\btheta}\Vert}{8} \right )\Phi^c(1) -\frac{3}{2}\left(\frac{1}{0.16^2}+\frac{1}{0.16} \sqrt{\frac{2}{\pi}} \right)\geq 1\label{eq:high_noise_lastprop_101},
\end{align}
where the first inequality follows from  Lemma~\ref{lem: logistic_case_2} (Note: $\bxi_k$ and $\btheta_{k-1}$ are independent). In the second inequality, we used that $\rho_{k-1}<\tfrac{3}{\sigma^2}$ and also the assumption that $0.16\Vert \bmu \Vert \leq \sigma$. The last inequality follows from the assumption that $\sigma \Vert\tilde{\btheta}_{k-1}\Vert\geq c$.  We therefore have 
\[
f(\btheta_{k-1})-f(\btheta^*)=\underbrace{f(\btheta_{k-1})-f(\rho_{k-1}\bmu)}_{\geq 1 \text{ by \eqref{eq:high_noise_lastprop_101}}}+\underbrace{f(\rho_{k-1}\bmu)-f(\btheta^*)}_{\geq 0 \text{ by Lemma~\ref{lem: logistic_case_1}}} \geq 1.
\]
We have thus shown \eqref{eq:high_thetak}. By Lemma~\ref{lem:technical_convex_bound}, we have 
  \begin{align} 
       f(\bm{\theta}_{k-1})-f(\bm{\theta}^*)&\leq \tfrac{1}{2\alpha}\left(\Vert  \bm{\theta}_{k-1}-\bm{\theta}^* \Vert^2-\bE\left[\Vert \bm{\theta}_{k}-\bm{\theta}^* \Vert^2\, |\mathcal{F}_{k-1}\right] \right)+\tfrac{\alpha}{2}\left (\norm{\bmu}^2 + d \sigma^2 \right ) \nonumber\\ &\leq \tfrac{1}{2\alpha}\left(\Vert  \bm{\theta}_{k-1}-\bm{\theta}^* \Vert^2-\bE\left[\Vert \bm{\theta}_{k}-\bm{\theta}^* \Vert^2\, |\mathcal{F}_{k-1}\right] \right)+\tfrac{1}{2}\min\{1,B\}, \label{eq:high_decrease_v2} 
    \end{align}
    where in the last inequality we used the assumption on $\alpha$, namely \eqref{eq:high_noise_alpha_assumption}. By \eqref{eq:high_thetak}, we obtain that 
\[
\min\{1,B\}\left(2\cdot 1_{\{\btheta_{k-1}\notin C\}}-1\right)\leq \tfrac{1}{\alpha}\left(\Vert  \bm{\theta}_{k-1}-\bm{\theta}^* \Vert^2-\bE\left(\Vert \bm{\theta}_{k}-\bm{\theta}^* \Vert^2\, |\mathcal{F}_{k-1}\right] \right).
\]
A simple manipulation then yields 
\begin{align}
    \bE\left[\overline{V}(\btheta_k)|\mathcal{F}_{k-1}\right] &\leq \overline{V}(\btheta_{k-1})-2\cdot 1_{\{\btheta_{k-1}\not\in {C} \}}+1 \nonumber \\&=\overline{V}(\btheta_{k-1})-1+2\cdot 1_{\{\btheta_{k-1}\in {C} \}}. \label{eq:high_noise_drift_eq}
\end{align}
From Appendix Lemma \ref{lem:drift_lemma_appendix}, we thus obtain that
\begin{equation}\label{eq:high_T_v2}
    \bE\left[\tau_m^{C}\right]\leq \overline{V}(\bm{0})+(m-1)\left(2+\sup_{\btheta\in {C}}\overline{V}(\btheta)\right).
\end{equation}
 It remains to upper bound the quantity $\sup_{\btheta\in {c}}\overline{V}(\btheta)$.  For any $\btheta \in C$, it holds that $\vert \rho\sigma^2-2\vert<1$. From this, we obtain that 
\begin{align*}
    \Vert \btheta-\btheta^*\Vert^2&=\left( \rho \sigma^2-\rho^*\sigma^2 \right )^2\frac{\Vert \bmu \Vert^2}{\sigma^4}+\Vert \tilde{\btheta}\Vert^2 \\&\leq \frac{\Vert \bmu \Vert^2}{\sigma^4}+\frac{c}{\sigma^2},
\end{align*}
We, therefore, have
\begin{equation}
    \sup_{\btheta\in {C}}\overline{V}(\btheta)\leq \frac{\Vert \bmu \Vert^2+c\sigma^2}{\alpha \sigma^4\min\{1,B\}}.
\end{equation}
The proof is complete. 
\end{proof}
We are now ready to prove Theorem~\ref{thm.b}.
\begin{proof}[Proof of Theorem \ref{thm.b}]
It follows from Proposition~\ref{prp:high_V} that there exists some constant $r>0$ such that $\bE\left[\tau_m^{C}\right]\leq rm$ for all $m\geq 1$. Taken Lemma~\ref{lem:st_ETC} and Lemma~\ref{lem: high_noise_delta} together, we obtain that
\[
\bE[T]\leq \bE[T_C]\leq \sum_{m=1}^{\infty}\bE[\tau_m^{C}]\Phi^{c}\left(\frac{-\sigma}{\Vert \bmu \Vert}\right)^{m-1}.
\]
Therefore, 
\[
\bE[T]\leq \bE[T_C]\leq r\sum_{m=1}^{\infty}m\Phi^{c}\left(\frac{-\sigma}{\Vert \bmu \Vert}\right)^{m-1}<+\infty.
\]
The proof is complete.
\end{proof}



